Quantum Error Correction with the GKP Code and Concatenation with Stabilizer Codes

Gottesman, Kitaev and Preskill have proposed a scheme to encode a qubit in a harmonic oscillator, which is called the GKP code. It is designed to be resistant to small shift errors contained in momentum and position quadratures. Thus there's some intrinsic fault tolerance of the GKP code. In this thesis,we propose a method to utilize all the information contained in the continuous shifts, not just simply map a GKP-encoded qubit to a normal qubit. This method enables us to do maximum-likelihood decisions and thus increase fault-tolerance of the GKP code. This thesis shows that the continuous nature of the GKP code is quite useful for quantum error correction.

==> Background/EncodingScheme.tex <==
\section{Encoding Scheme of GKP Code States}
\label{sec:encoding_oscillator}

In this section, we discuss the encoding scheme of the GKP code states introduced by Gottesman \textit{et al.} \cite{gottesman2001encoding} in order to protect a state of a finite dimensional quantum system that isencoded in an infinite-dimensional system, i.e. encoding a qubit into a harmonic oscillator.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Encoding a Qubit in an $d$-Dimensional System}

Gottesman \textit{et al.}\ first developed a kind of higher-dimensional error correction code \cite{gottesman2001encoding}, where the Pauli operators are generalized to be:
\begin{align*}
X: \ket{j} &\to \ket{(j + 1) \ \text{mod}\ d},\\
Z: \ket{j} &\to \omega \ket{j},\\
[X,Z] &= (1-\omega)XZ,
\end{align*}
where $d$ is the dimension of the system and $\omega = e^{ 2 \pi \mathrm{i} /d}$. In order to protect the qubit from the action of small powers of these operators called ```shifts'', the generators of the stabilizer group are defined to be:
\begin{align}
S_X = X^{2 r_1}, \,\, S_Z = Z^{2 r_2}
\label{eq:GKP_stabilizer}
\end{align}
where the dimension of the system is $d = 2 r_1 r_2$.
The logical operators are thus defined as:
\begin{align*}
\bar{X} = X^{r_1}, \,\, \bar{Z} = Z^{r_2}.
\end{align*}
The stabilizers commute with a generalized Pauli operator $X^a Z^b$ if both $a$ and $b$ are integer multiples of $r_1$ and $r_2$ respectively, thus the stabilizers cannot distinguish he states $\ket{\bar{\Psi}}$ and $\bar{P}\ket{\bar{\Psi}}$, where $\bar{P}$ is some logical Pauli operator, and $\ket{\bar{\Psi}}$ any encoded code state.  So shifts can be corrected perfectly if:
\begin{align*}
|a|, |b| <\frac{r_1}{2}
\end{align*}
The basis states (logical $\ket{0}$ and logical $\ket{1}$) of this code are:
\begin{align*}
\ket{\bar{0}} &= \frac{1}{\sqrt{r_1}}(\ket{0} + \ket{2 r_1} + \dots + \ket{2(r_2-1)r_1}),\\
\ket{\bar{1}} &= \frac{1}{\sqrt{r_1}}(\ket{r_1} + \ket{3 r_1} + \dots + \ket{(2(r_2-1)+1)r_1}).
\end{align*}

\subsubsection{Qubit in an 18-Dimensional System}
Here we consider a qubit encoded into an $18$-dimensional system as an example.  In this case we set $r_1 = r_2 = 3$, which leads to :
\begin{align*}
&S_X = X^6,  &S_Z=Z^6\\
&\bar{X} = X^3,  &\bar{Z} = Z^3.
\end{align*}
and basis states (logical $\ket{0}$ and logical $\ket{1}$):
\begin{align*}
\ket{\bar{0}} &= \frac{1}{\sqrt{3}}(\ket{0}+\ket{6}+\ket{12}),\\
\ket{\bar{1}} &= \frac{1}{\sqrt{3}}(\ket{3}+\ket{9}+\ket{15})
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Encoding a Qubit in an Infinite-Dimensional System}
It's easy to generalize this code to an infinite-dimensional system, $d\to \infty$. For simplicity we keep $d = 2 r_1 r_2 \equiv  1/\epsilon^2$ and $r_1 \equiv \alpha/ \epsilon$, which leads to $r_2 = 1/(2 \epsilon \alpha)$ where $\epsilon$ is infinitesimally small ($\epsilon \to 0)$. Now a natural generalization of the qudit is to associate the basis $\{\ket{j}\}$ of the qudit with the position basis $\ket{q}$ and the phase with the momentum basis $\ket{p}$ of a harmonic oscillator. The generalized Pauli operators can be written as shifts in position or momentum:
\begin{align*}
Z \to e^{2 \pi i \hat{q} \epsilon}, \qquad   X \to e^{-i \hat{p} \epsilon}.
\end{align*}
Thus, the stabilizers in Eq.(\ref{eq:GKP_stabilizer}) are given by:
\begin{align*}
& S_{\hat{q}} = Z^{2r_2} = Z^{1/(\alpha \epsilon)} = e^{2 \pi i \hat{q}/\alpha}\\
& S_{\hat{p}} = X^{2r_1} = X^{2 \alpha/\epsilon}   = e^{-2 i \hat{p} \alpha}
\end{align*}
The space fixed by $S_{\hat{q}}$ and $S_{\hat{p}}$ is two dimensional as there are additional operators which we can identify the logical operators as:
\begin{equation*}
\bar{Z} = e^{\pi i \hat{q}/\alpha}, \qquad \bar{X} = e^{- i \hat{p} \alpha}
\end{equation*}
where $\alpha$ is some real parameter. Using the identity $e^{A}e^{B} = e^{[A,B]}e^{B}e^{A}$(which holds if A and B commute with their commutator) and the canonical commutation relation $[q,p] = i$, we verify that:
\begin{equation*}
\bar{Z} \bar{X} = \omega \bar{X} \bar{Z}, \quad \omega = e^{\pi i}
\end{equation*}
The condition  $S_{\hat{q}}=1$ and $S_{\hat{p}}=1$ fixes the both momentum $p=0 \mod \sqrt{\pi}$ and position $q=0 \mod \sqrt{\pi}$ to be sharply determined. Since $\bar{X}$ translates $q$ by $\alpha$ and $\bar{Z}$ translates $p$ by $\pi / \alpha$, then the code protects against shifts with:
\begin{equation*}
\vert \Delta q \vert < \frac{\alpha}{2}, \quad \vert \Delta p \vert < \frac{\pi}{2 \alpha}
\end{equation*}
Then a code state in this subspace thus escape Heisenberg's uncertainty principle by being not localized at a single $p$ and $q$. The shifts in momentum and position that the code can correct obey the condition:
\begin{align*}
\Delta q \Delta p < \frac{\pi}{4} \hbar
\end{align*}
Note that the stabilizer operators $S_{\hat{p}},S_{\hat{q}}$ are not the only generators of the stabilizer group. In order to generate the whole group, the Hermitian conjugate of them are needed as well.
Although they are not Hermitian themselves, their actions on the code space are equivalent to the action of their Hermitian conjugate.
The $\ket{\bar{0}},\ket{\bar{1}}$ ($\ket{\bar{+}}, \ket{\bar{-}}$) states are the $\pm 1$ eigenstates of $\bar{Z}$ ($\bar{X}$):
\begin{align}
&\ket{\bar{0}} = \sum_{s=-\infty}^{\infty}\ket{q=2 s \alpha}, &&\ket{\bar{+}} = \sum_{s=-\infty}^{\infty}\ket{p=2 s\pi/ \alpha},\\
&\ket{\bar{1}} = \sum_{s=-\infty}^{\infty}\ket{q=(2s +1) \alpha}, &&\ket{\bar{-}} = \sum_{s=-\infty}^{\infty}\ket{p=(2 s+1)\pi / \alpha}.
\label[pluralequation]{eq:perfect_code_word}
\end{align}
The wavefunction is shown in \cref{fig:ideal_code_states}, where we set $\alpha=\sqrt{\pi}$ to assure the code state to be symmetric in both quadratures:
\begin{equation}
\bar{Z} = e^{ i\sqrt{\pi} \hat{q}}, \qquad \bar{X} = e^{- i \sqrt{\pi} \hat{p} }
\label{eq:symmetric_q_p}
\end{equation}
Also the errors in $q$ and $p$ quadratures are now of comparable magnitude. One can easily check that the logical operators perform the desired action on the code space and the stabilizers $S_{\hat{p}}$ and $S_{\hat{q}}$ both map any code state back to itself.


\begin{figure}
\centering
\subfigure[][]{
\begin{minipage}{\textwidth}
\begin{minipage}{.1\textwidth}
$\ket{\bar{0}} = $
\end{minipage}
\begin{minipage}{.8\textwidth}
\includegraphics[width=\textwidth]{Background/ideal_codeword_0_q.png}
\end{minipage}
\hfill
\end{minipage}}\\
\subfigure[][]{
\begin{minipage}{\textwidth}
\begin{minipage}{.1\textwidth}
$\ket{\bar{1}} = $
\end{minipage}
\begin{minipage}{.8\textwidth}
\includegraphics[width=\textwidth]{Background/ideal_codeword_1_q.png}
\end{minipage}
\hfill
\end{minipage}}
\caption[The ideal code states $\ket{\bar{0}}$ and $\ket{\bar{1}}$ in the $\hat{q}$ quadrature]{The ideal code states $\ket{\bar{0}}$ and $\ket{\bar{1}}$ in the $\hat{q}$ quadrature for $\alpha=\sqrt{\pi}$. It's easy to see that the ideal states are composed of $\delta$ functions, which requires infinite squeezing. So the states are unphysical, it can also be seen that the wave function of these states are not normalizable.}
\label{fig:ideal_code_states}
\end{figure}









==> tex/list_of_symbols.tex <==
\chapter*{List of Symbols}
\addcontentsline{toc}{chapter}{List of Symbols}

\begin{longtable}[l]{p{120pt} p{300pt}}
\textbf{\large Symbol}	& \textbf{\large Description} \\
& \\
$\ket{\bar{0}}$, $\ket{\bar{1}}$, $\ket{\bar{+}}$, $\ket{\bar{-}}$ 
& encoded qubit states 0,1 and $+$,$-$\\
$\ket{\tilde{0}}$, $\ket{\tilde{1}}$, $\ket{\tilde{+}}$, $\ket{\tilde{-}}$ & approximate qubit states 0,1 and $+$,$-$\\
$\ket{\alpha}$	& coherent state\\
$a$				& annihilation operator\\
$a^\dag$		& creation operator\\
$\delta_{nm}$	& Kronecker delta\\
$\delta(\cdot)$	& Dirac delta distribution\\
$\Delta$		& Squeezing parameter of approximate code states\\
$\Delta_H$		& detuning $\omega_r-\omega_q$\\
$D(\cdot)$		& displacement operator\\
$\hat{n}$		& photon number operator\\
$\ket{n}$		& Fock state\\
$\hat{p}$		& momentum quadrature operator\\
$\ket{p}$		& eigenstate of $\hat{p}$\\
$p$				& eigenvalue of the eigenstate $\ket{p}$ of $\hat{p}$\\
$\hat{q}$		& position quadrature operator\\
$\ket{q}$		& eigenstate of $\hat{q}$\\
$q$				& eigenvalue of the eigenstate $\ket{q}$ of $\hat{q}$\\
$S_{\hat{p}}$	& stabilizer of the code space for the p quadrature\\
$S_{\hat{q}}$	& stabilizer of the code space for the q quadrature\\
$\ket{u,v}$	    & shifted code state \\
$\ket{u,v}_q$	& shifted code state in $\hat{q}$ quadrature\\
$\ket{u,v}_p$	& shifted code state in $\hat{p}$ quadrature\\
$X$				& (generalized) Pauli $X$\\
$\bar{X}$		& logical Pauli $X$ in the GKP code\\
$Z$				& (generalized) Pauli $Z$\\
$\bar{Z}$		& logical Pauli $Z$ in the GKP code\\
& \\
& \\
& \\
& \\
& \\
& \\& \\
& \\
\textbf{\large Abbreviation}	& \textbf{\large Description} \\
& \\
MLD			    & Maximum-Likelihood Decoding\\
MWM    	        & Minimum-Weight Perfect Matching\\
CNOT gate		& Controlled NOT Gate \\
CPHASE gate		& Controlled Phase Gate\\\
GKP	code		& Code Proposed by Gottesman, Kitaev and Preskill\\


\end{longtable}

